Does Video Compression Impact Tracking Accuracy?

Everyone "knows" that compressing a video will degrade the accuracy of object tracking. Yet, a literature search on this topic reveals that there is very little documented evidence for this presumed fact. Part of the reason is that, until recently, there were no object tracking datasets for uncompressed video, which made studying the effects of compression on tracking accuracy difficult. In this paper, using a recently published dataset that contains tracking annotations for uncompressed videos, we examined the degradation of tracking accuracy due to video compression using rigorous statistical methods. Specifically, we examined the impact of quantization parameter (QP) and motion search range (MSR) on Multiple Object Tracking Accuracy (MOTA). The results show that QP impacts MOTA at the 95% confidence level, while there is insufficient evidence to claim that MSR impacts MOTA. Moreover, regression analysis allows us to derive a quantitative relationship between MOTA and QP for the specific tracker used in the experiments.

==> tables/sequence_list.tex <==
\begin{table}[!htbp]
    \centering
    \caption[List of ground truths for the uncompressed video sequences]
    {List of ground truths for the uncompressed video sequences adapted from \cite{SFU-HW-Tracks-v1}.}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{|| c | c | c | c | c | c | c ||}
         \hline
          Sequence Class & Sequence Name & Frame Count & Resolution & Object Class IDs & Frame rate (Hz) & Bit depth  \\ [0.5ex]
         \hline\hline
          B & BasketballDrive & 500 & 1920x1080 & [0, 32, 56] & 50 & 8 \\ 
         \hline
          B & Cactus & 500 & 1920x1080 & [58] & 50 & 8 \\ 
         \hline
          B & Kimono & 240 & 1920x1080 & [0, 26] & 24 & 8 \\
         \hline
          B & ParkScene & 240 & 1920x1080 & [0, 1, 13] & 24 & 8 \\
         \hline
          C & BasketballDrill & 500 & 832x480 & [0, 32, 56] & 50 & 8 \\
         \hline
          C & PartyScene & 500 & 832x480 & [0, 41, 58, 74, 77] & 50 & 8 \\
         \hline
          C & RaceHorsesC & 300 & 832x480 & [0, 17] & 30 & 8 \\
         \hline
          D & BasketballPass & 500 & 416x240 & [0, 32, 56] & 50 & 8 \\
         \hline
          D & BlowingBubbles & 500 & 416x240 & [0, 41, 77] & 50 & 8 \\
          \hline
          D & RaceHorsesD & 500 & 416x240 & [0, 17] & 30 & 8 \\
          \hline
          E & KristenAndSara & 600 & 1280x720 & [0, 63, 67] & 60 & 8 \\
          \hline
          E & Johnny & 600 & 1280x720 & [0, 27, 63] & 60 & 8 \\
          \hline
          E & FourPeople & 600 & 1280x720 & [0, 41, 56, 58] & 60 & 8 \\
          \hline
    \end{tabular}
    }
    \label{tab:sequence_list}
\end{table}
% \vspace{-0.3cm}
